Reflective Gaussian Splatting

Novel view synthesis has experienced significant advancements owing to increasingly capable NeRF- and 3DGS-based methods. However, reflective object reconstruction remains challenging, lacking a proper solution to achieve real-time, high-quality rendering while accommodating inter-reflection. To fill this gap, we introduce a Reflective Gaussian splatting (Ref-Gaussian) framework characterized with two components: (I) Physically based deferred rendering that empowers the rendering equation with pixel-level material properties via formulating split-sum approximation; (II) Gaussian-grounded inter-reflection that realizes the desired inter-reflection function within a Gaussian splatting paradigm for the first time. To enhance geometry modeling, we further introduce material-aware normal propagation and an initial per-Gaussian shading stage, along with 2D Gaussian primitives. Extensive experiments on standard datasets demonstrate that Ref-Gaussian surpasses existing approaches in terms of quantitative metrics, visual quality, and compute efficiency. Further, we show that our method serves as a unified solution for both reflective and non-reflective scenes, going beyond the previous alternatives focusing on only reflective scenes. Also, we illustrate that Ref-Gaussian supports more applications such as relighting and editing.

==> tables/ablation_mae_re.tex <==
\begin{table*}[!h]
\centering

\caption{Comparison of MAE values across different models.}
\label{tb:mae_comparison_re}
\vspace{0.1cm} 

\resizebox{0.3\textwidth}{!}{
\begin{tabular}{l|c}
\hline
\hline
\textbf{Model} & \textbf{MAE (avg)} \\
\hline
\textbf{\textbf{\model{}}} & \cellcolor{red!50}2.15 \\
\textbf{w/o 2DGS} & 5.04 \\
\textbf{w/o Initial stage} & \cellcolor{red!10}3.53 \\
\textbf{w/o Material-aware} & 3.86 \\
\textbf{w/o PBR} & 3.81 \\
\hline
\hline
\end{tabular}
}
\end{table*}


==> tables/ablation_re.tex <==
\begin{table*}[!h]
\centering

\caption{Ablation studies on the components of \model{}. w/o Material-aware: use original normal propagation following 3DGS-DR~\citep{ye20243d}.}
\label{tb:ablation_2D_re}
\vspace{0.3cm} 
\renewcommand{\arraystretch}{1.2}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{l|c|c|c|c|c|c|c}
\hline
\hline

\textbf{Model} & {\textbf{\model{}}} & {\textbf{w/o PBR}} & {\textbf{w/o Inter-reflection}} & {\textbf{w/o 2DGS}}  & {\textbf{w/o Deferred rendering}} & {\textbf{w/o Initial stage}} & {\textbf{w/o Material-aware}} \\
\hline

\textbf{PSNR$\uparrow$} & \cellcolor{red!50}30.33 & 29.84 & \cellcolor{red!10}30.14 & 28.93 & 28.85 & 29.94 & 29.68 \\
\textbf{SSIM$\uparrow$} & \cellcolor{red!50}0.958 & 0.956 & \cellcolor{red!10}0.957 & 0.935 & 0.935 & 0.956 & 0.952 \\
\textbf{LPIPS$\downarrow$} & \cellcolor{red!50}0.049 & 0.052 & \cellcolor{red!10}0.050 & 0.071 & 0.074 & 0.052 & 0.056 \\
\hline
\hline
\end{tabular}
}
\end{table*}


